Data-Driven Analysis to Understand GPU Hardware Resource Usage of Optimizations

With heterogeneous systems, the number of GPUs per chip increases to provide computational capabilities for solving science at a nanoscopic scale. However, low utilization for single GPUs defies the need to invest more money for expensive ccelerators. While related work develops optimizations for improving application performance, none studies how these optimizations impact hardware resource usage or the average GPU utilization. This paper takes a data-driven analysis approach in addressing this gap by (1) characterizing how hardware resource usage affects device utilization, execution time, or both, (2) presenting a multi-objective metric to identify important application-device interactions that can be optimized to improve device utilization and application performance jointly, (3) studying hardware resource usage behaviors of several optimizations for a benchmark application, and finally (4) identifying optimization opportunities for several scientific proxy applications based on their hardware resource usage behaviors. Furthermore, we demonstrate the applicability of our methodology by applying the identified optimizations to a proxy application, which improves the execution time, device utilization and power consumption by up to 29.6%, 5.3% and 26.5% respectively.

==> analysis.tex <==
% Explain the analysis methodology. What are the features, what is the target. We are the research questions?
Adaptation of deep learning from grid-alike data (e.g. images) to graphs has recently received unprecedented attention from both machine learning and data mining communities, leading to a new cross-domain field---Deep Graph Learning (DGL). Instead of painstaking feature engineering, DGL aims to learn informative representations of graphs in an end-to-end manner. It has exhibited remarkable success in various tasks, such as node/graph classification, link prediction, etc~\cite{yu2020deep}. 
Deep graph-learning is a the application areas where deep graph-learning has been traditionally applied are to analyze medical and social network structures to infer relationships among features. The domain knowledge of these applications clearly describe what each node, edge, and edge-weights of a graph mean. However, the same is not true for application performance. To the best of our knowledge, no work in the literature has modeled application performance as a graph. Hence, in this paper, we investigate different ways to build the graph and leverage unsupervised graph learning algorithms to automatically learn the latent correlations across different performance profiles of applications as under different conditions (e.g., different input parameters and control frequencies) and evaluate their effectiveness in conducting the important task of performance prediction for HPC applications. The following sections describe each step in the process in details.
%Why this new approach?
\subsection{Motivation for Formulating Performance as a Graph}
The motivation for investigating this new approach is to both advance the area of HPC performance analytics by leveraging extremely powerful unsupervised learning techniques that can automatically discern patterns based on similarities at high dimensions than what a linear supervised neural network or manual investigation can identify. These learned features then can serve as the representations of salient characteristics to downstream machine learning tasks of regression or classification to solve challenging HPC problems such as performance prediction on new architectures and comparison across different architectures. Also, this new approach of graph representation learning can be used to generate new performance profiles by further adapting techniques such as GraphGAN~\cite{wang2017graphgan}. Hence, research presented in this paper builds the foundation for a new avenue in the area of HPC performance data analytics. Also, once a graph is built, that means other approaches such as community detection can be mapped to identifying correlated performance counters, within the same system, across systems can be pursue. New problem areas will emerge with the success of this research approach. Others may investigate this avenue of research further and we may have a solution that works on challenging HPC performance problems. 
% The rationale is that even though architectures are widely different and will continue to evolve (e.g., CPUs, GPUs, accelerators, FPGAs, and wafer-scale), they share common core units such as compute units (e.g., scalar, vector, axiliary processing units, floating-point processing units), cache layers (e.g., L1, L2, L3 in CPUs, texture cache, global cache, shared cache in GPUs), memory (e.g., global, system, remote), instruction unit. So, even though the low-level performance counters may have different names and no similarity across architectures, there may exist similarity in how an application interacts with the texture cache on one GPU vs the shared cache on another GPU on a different vendor. Manually investigating performance profiles across different architectures is infeasible. So to investigate

\subsection{Graph Representation Learning is Challenging}
The central problem in machine learning on graphs is finding a way to incorporate information about graph-structure into a machine learning model. For example, in the case of link prediction in a social network, one might want to encode pairwise properties between nodes, such as relationship strength or the number of common friends. Or in the case of node classification, one might want to include information about the global position of a node in the graph or the structure of the node’s local graph neighborhood (Figure 1). The challenge— from a machine learning perspective—is that there is no straightforward way to encode this high-dimensional, non-Euclidean information about graph structure into a feature vector.

To extract structural information from graphs, traditional machine approaches often rely on summary graph statistics (e.g., degrees or clustering coefficients) [6], kernel functions [58], or carefully engineered features to measure local neighborhood structures [40]. However, these approaches are limited because these hand- engineered features are inflexible—i.e., they cannot adapt during the learning process—and designing these features can be a time-consuming and expensive process. Specifically, for performance data, none of these ideas make sense. 

More recently, there has been a surge of approaches that seek to learn representations that encode structural information about the graph. The idea behind these representation learning approaches is to learn a mapping that embeds nodes, or entire (sub)graphs, as points in a low-dimensional vector space Rd. The goal is to optimize this mapping so that geometric relationships in the embedding space reflect the structure of the original graph. After optimizing the embedding space, the learned embeddings can be used as feature inputs for downstream machine learning tasks. The key distinction between representation learning approaches and previous work is how they treat the problem of representing graph structure. Previous work treated this problem as a pre-processing step, using hand-engineered statistics to extract structural information. In contrast, representation learning approaches treat this problem as machine learning task itself, using a data-driven approach to learn embeddings that encode graph structure.

While there are many disparate lines of research that have drawn significant attention across different subfield and venues in recent years, we specifically investigate the node embedding method, which are popular object of study in the data mining community, and graph convolutional networks, which have drawn considerable attention in major machine learning venues. 
% In Section~\ref{sec:analysis} we proposed different approaches of building the graph, creating edges, and computing weights both using simple distance measures and by leveraging sophisticated learning techniques.

\subsection{Building Performance Graph}
% Graph representation learning is an unsupervised learning technique for automatically identifying correlations across several 
Learning graph representations is a fundamental task aimed at capturing various properties of graphs in vector space. 
% % The most recent methods learn such representations for static networks.
% From high-level, in this paper, we propose to map application performance collected under hundreds of configurations to the nodes of an undirected graph $G = {V, E}$, where $V$ is the set of nodes representing each configuration, $E$ represents the set of edges between each node, with associated binary adjacency matrix $A$.
Mathematically, the input to our representation learning algorithm is an undirected graph $G = (V,E)$ with associated binary adjacency matrix $A$. Here, $V$ represents the set of nodes where each node maps to performance data collected under a certain configuration (e.g., various inputs, control frequencies, power cap). Each node contains a real-valued vector of performance attributes $X \in R^{m}$ (e.g., $m$ number of hardware performance counters). The goal of the graph representation learning methodology is to use the information contained in $A$ and $X$ to map each node, or a subgraph, to a vector $z \in R^{d}$, where $d << |V|$. In this research, we investigate two methods of providing $A$ to the representation learning algorithm, where in one approach we build $A$ by using an Eucledian measure for computing high-dimensional distance. In the second approach, we build random embeddings and let the learning algorithm ``figure" out the relationships and weights automatically. Section~\ref{sec:results} evaluates both approaches from their effectiveness in conducting the supervised task of performance prediction. 
% weights to represent similarity between two configurations based on certain measure. The intuitive rationale for this novel analysis methodology is that it is possible to ``travel" from one node (configuration) to another node in a performance graph by changing one or more operating condition (e.g., input, runtime parameters, number of tasks, power cap, control frequency). 

Most of the methods we review will optimize this mapping in an unsupervised manner, making use of only information in A and X, without knowledge of a particular downstream machine learning task. 

% These representations can be improved further by takingHowever, we will also discuss some approaches for supervised representation learning, where the models make use of classification or regression labels in order to optimize the embeddings. These classification labels may be associated with individual nodes or entire subgraphs and are the prediction targets for downstream machine learning tasks (e.g., they might label protein roles, or the therapeutic properties of a molecule, based on its graph representation).
% 2Most of the methods we review are easily generalized to work with weighted or directed graphs, and we will explicitly describe how to generalize certain methods to the multi-modal setting (i.e., differing node and edge types).
% with associated binary adjacency matrix A.
% matrix of node attributes X ∈ Rm×|V| (e.g., representing text or metadata associated with nodes). The goal is to use the information contained in A and X to map each node, or a subgraph, to a vector z ∈ Rd, where d << |V|.

%\subsection{Learning Unsupervised Graph Representation}
% From high-level, in this paper, we propose to map application performance collected under hundreds of configurations to a graph, where nodes represent each configuration, edges represent their relationship under certain function, and weights to represent similarity between two configurations based on certain measure. The intuitive rationale for this novel analysis methodology is that it is possible to ``travel" from one node (configuration) to another node in a performance graph by changing one or more operating condition (e.g., input, runtime parameters, number of tasks, power cap, control frequency). In Section~\ref{sec:analysis} we proposed different approaches of building the graph, creating edges, and computing weights both using simple distance measures and by leveraging sophisticated learning techniques.

% To the best of our knowledge, there exists no work that takes a similar approach. 

% In this tutorial, we aim to provide a comprehensive introduction to deep graph learning. We first introduce the theoretical foundations on deep graph learning with a focus on describing various Graph Neural Network Models (GNNs). We then cover the key achievements of DGL in recent years. Specifically, we discuss the four topics: 1) training deep GNNs; 2) robustness of GNNs; 3) scalability of GNNs; and 4) self-supervised and unsupervised learning of GNNs. Finally, we will introduce the applications of DGL towards various domains, including but not limited to drug discovery, computer vision, medical image analysis, social network analysis, natural language processing and recommendation.

% Deep graph-learning is a the application areas where deep graph-learning has been traditionally applied are to analyze medical and social network structures to infer relationships among features. The domain knowledge of these applications clearly describe what each node, edge, and edge-weights of a graph mean. However, the same is not true for application performance. 


==> avgLossSmUtil.tex <==
The objective of this analysis is to identify which resource utilization behaviors can explain the loss of GPU utilization. Since the goal is to understand how to improve the system utilization of GPUs, we use $1 - normalized\_average\_sm\_utilization$ (utilization loss) and identify the resource groups and the performance events that are non-negatively correlated with this target. Table~\ref{tab:app-configs} describes the input parameters that are used to run these applications. 

The observations that can be made are:
\begin{itemize}
    \item In Figure~\ref{fig:sunburst-util-loss}a, the average loss of utilization for all three regions (\texttt{lt}, \texttt{lplust}, and \texttt{sweep}) in Kripke can be explained by the number of system memory write requests to the L2 cache. The same event is also a strong indicator of the average power usage of Kripke, which means, that reducing the number of system memory write requests to the L2 cache for Kripke will improve both the power usage (reduce) and the device utilization (increase). Similar observation also applies to Pennant, which means similar optimizations can be applied to both of the applications to improve power usage and device utilization.
    
    \item In Figure~\ref{fig:sunburst-util-loss}b, gpuMain2 and gpuMain4 kernels in Pennant have bank conflicts also as strong indicators of average loss of utilization, similar to its power usage behavior. This indicates that the same optimization for changing the memory access pattern of application to reduce bank conflict will also improve (reduce) the power usage as well as the device utilization of Pennant.
    
    \item In Figure~\ref{fig:sunburst-util-loss}b, gpuMain2 and gpuMain4 kernels in Pennant have bank conflicts also as strong indicators of average loss of utilization, similar to its power usage behavior. This indicates that the same optimization for changing the memory access pattern of application to reduce bank conflict will also improve (reduce) the power usage as well as the device utilization of Pennant.

    \item In Figure~\ref{fig:sunburst-util-loss}c, the \texttt{dot\_kernel} remains memory bound regardless of the change in frequency. This indicates that the kernel does not have enough computation and might benefit from the memory access optimization regardless of the computation frequency. 
    
    % \item In Figure~\ref{fig:sunburst-util-loss}c, among the 23 kernels, the \texttt{device\_ideal\_gas\_kernel\_cuda} kernel has the largest utilization loss. By focusing on the resource utilization behaviors that can explain utilization loss (Figure~\ref{fig:sunburst-util-loss}d), we find that the number of write requests to the Texture cache of the L2 cache explains utilization loss for Cloverleaf. To be specific, 48\% of the behavior of utilization loss across several iterations of Cloverleaf using different input parameters and different execution frequencies can be explained by the number of write requests to the L2-Texture cache. Hence, reducing the number of such requests will also reduce the loss of utilization (hence improve device utilization) for Cloverleaf. 
\end{itemize}


==> avgpower.tex <==
The objective of this analysis is to identify which resource utilization behaviors explain the average power usage of applications on a GPU. Since the goal is to understand the existing application's behaviors, we set the NVML metric 'average power usage' as the target in \pipeline and all of the CUPTI events as the features. Table~\ref{tab:app-configs} describes the input parameters that are used to run these applications. 

From Figure~\ref{fig:sunburst-power} we can observe that:
\begin{itemize}
    \item In Figure~\ref{fig:sunburst-power}a, the average power usage of all three regions (\texttt{lt}, \texttt{lplust}, and \texttt{sweep}) can be explained by their utilization of the L2\_P0 resource group. Specifically, out of \change{XX} performance events in this group, the l2\_subp0\_write\_sysmem\_sector\_queries event dominantly explains the average power usage behavior of Kripke. This performance event counts the number of system memory write requests made to slice 0 of L2 cache. This increments by 1 for each 32-byte access. This performance event exposes that due to a large number of write requests from the system memory to the L2 cache, Kripke consumes more average power. This observation is supported by a similar finding in the literature~\cite{allen2016characterizing} that GPU memory access consumes more power than CPU memory access. 
    In Figure~\ref{fig:sunburst-power}b, the number of write requests from the system memory to the slide 1 of L2 cache strongly explains the average power usage of Pennant (all groups). 
    \item In Figure~\ref{fig:sunburst-power}b, the number of shared bank conflict generated when the addresses for two or more shared memory requests fall in the same memory bank. The average power usage of kernel \texttt{gpuMain2} is dominated by the bank conflicts during the load operations from the shared memory, whereas that of the kernel \texttt{gpuMain4} is dominated by the bank conflicts generated during the store operations. 
\end{itemize}

Ge et. al.~\cite{allen2016characterizing} show that system memory accesses to the L2 cache consumes power. In general, we have observed that the system memory write event to any slice of the L2 cache explains a significant portion of the average power usage across several applications running with several inputs. This observation indicates that to reduce the average power usage of an application, a good starting point would be to reduce the number of write operations to the L2 cache of GPUs. \hl{But how? Could we at least find a reference that talks about optimizations for reducing the number of system memory write operations to the L2 cache? Buffering? Caching? What?}%%But how?
% Since the number of these accesses strongly correlate with the average power usage of application on Nvidia Volta, 
Bank conflict can be optimized by changing the memory access pattern. \hl{Any example with respect to Pennant?}

==> kripke.tex <==

\subsection{Kripke}

\begin{figure*}[htbp]
\centering
    {\includegraphics[width=\textwidth]{figs/kripke_large.pdf}
  \caption{Kripke}
  \label{fig:kripke}
}
\end{figure*}
In this section, we present the resource utilization behaviors of three annotated regions--\texttt{esweep, elt, and elplust} in \kripke that make up the majority of the physics of an SN transport application. \kripke provides six striding orders of Directions (D), Groups (G), and Zones (Z), and provides computational kernels specifically written for each of these nestings. In this paper, we compare two nesting orders DGZ and DZG to identify which nesting order utilizes hardware resources better and how their performance compares. Figure~\ref{fig:kripke}a presents two resource utilization behaviors of the DGZ and DZG loop nesting orders. From Figure~\ref{fig:kripke}b we can observe that the computational resource utilization behavior of the DGZ loop nesting order explains the optimal trade off between utilization and execution performance on Nvidia Volta compared to the DGZ nesting order. Figure~\ref{fig:kripke}b presents the change in both performance and device utilization of DZG compared to DGZ. We can observe that the score metric (blue solid line) emulates the utilization curve better when the change in execution time is small, but gets heavily penalized (low value) when the execution time increases (poor performance). Figure~\ref{fig:kripke}c presents the comparative bar chart that presents the change in resource usage behavior between DZG and DGZ to explain the change in score behavior (the set of performance events that can construct the blue solid line in Figure~\ref{fig:kripke}b). From Figure~\ref{fig:kripke}a and~\ref{fig:kripke}c, we can again observe that comparative analysis using the differential method identifies how the two nesting orders utilized different hardware resources and which hardware resource usage jointly contributed to the change in both device utilization and execution time. Specifically, we observe that the DZG kernel utilizes the compute resources (FMA and FP64) more than DGZ nesting, this behavior caused DZG to obtain more device utilization (Figure~\ref{fig:kripke}b) with only small difference in the average execution time. This analysis, with a real application, demonstrates that comparative analysis with the proposed target metric can help application scientists, performance analysts, and facilities to identify suitable implementation of the same application that can improve device utilization at the cost of no application performance degradation or both.

% Figure~\ref{fig:sunburst-kripke}a shows the high-level insights about the resource utilization behaviors of each kernel that lead to the average power usage during the run of each kernel,~\ref{fig:sunburst-kripke}b provides the resource utilization behaviors that can explain the loss of average sm utilization, and~\ref{fig:sunburst-kripke}c shows the resource utilization behaviors that can explain the achieved trade-off between device utilization and application performance.

% All regions, resources, and events are sorted based on their values (e.g., percent average sm utilization, importance) and organized in counter-clockwise manner.

% The observations that can be made from Figure~\ref{fig:sunburst-kripke} are:
% \begin{itemize}
%     \item Which resources are correlated with the average power usage?
%     \item Which resources are correlated with the average utilization loss?
%     \item Which resources or events are correlated with the best trade-off? 
% \end{itemize}

==> new.tex <==
@misc{top500,
  title={Top500 List of Supercomputers},
  howpublished={\url{https://www.top500.org/lists/top500/2023/11/}},
  author={Strohmaier, Erich and Dongarra, Jack and Simon, Horst and Meuer, Martin}
}

@mastersthesis{ye2009design,
    author = {Ye, Zhenyu},
    title = {Design Space Exploration for GPU-Based Architecture},
    school = {Eindhoven University of Technology},
    year = {2009},
}

@inproceedings{islam2016a,
  title={A machine learning framework for performance coverage analysis of proxy applications},
  author={Islam, Tanzima Z and Thiagarajan, Jayaraman J and Bhatele, Abhinav and Schulz, Martin and Gamblin, Todd},
  booktitle={SC'16: Proceedings of the International Conference for High Performance Computing, Networking, Storage and Analysis},
  pages={538--549},
  year={2016},
  organization={IEEE}
}

@inproceedings{allen2016characterizing,
  title={Characterizing power and performance of GPU memory access},
  author={Allen, Tyler and Ge, Rong},
  booktitle={2016 4th International Workshop on Energy Efficient Supercomputing (E2SC)},
  pages={46--53},
  year={2016},
  organization={IEEE}
}

@article{ferenbaugh2015pennant, 
author = {Ferenbaugh, Charles R.}, 
title = {PENNANT: An Unstructured Mesh Mini-App for Advanced Architecture Research}, 
year = {2015}, 
issue_date = {December 2015}, 
publisher = {John Wiley and Sons Ltd.}, 
address = {GBR}, 
volume = {27}, 
number = {17}, 
issn = {1532-0626}, 
howpublished={\url{https://proxyapps.exascaleproject.org/pennant/}},
doi = {10.1002/cpe.3422}, 
abstract = {This paper describes PENNANT, a mini-app that operates on general unstructured meshes meshes with arbitrary polygons, and is designed for advanced architecture research. It contains mesh data structures and physics algorithms adapted from the Los Alamos National Laboratory radiation-hydrodynamics code FLAG and gives a sample of the typical memory access patterns of FLAG. The basic capabilities and optimization approaches of PENNANT are presented. Results are shown from sample performance experiments run on serial, multicore, and graphics processing unit implementations, giving an indication of how PENNANT can be a useful tool for studies of new architectures and programming models. Copyright © 2014 John Wiley & Sons, Ltd.},
journal = {Concurr. Comput.: Pract. Exper.},
month = {dec},
pages = {4555–4572},
numpages = {18},
keywords = {unstructured mesh, advanced architectures, Lagrangian hydrodynamics, multicore, GPU} 
}

@misc{minife,
  title={miniFE},
  howpublished={\url{https://github.com/Mantevo/miniFE}},
  author={Free Software Foundation Inc.},
  year={2007}
}

@article{mixbench,
    author = {Konstantinidis, Elias and Cotronis, Yiannis },
    title = {A quantitative roofline model for GPU kernel performance estimation using micro-benchmarks and hardware metric profiling},
    year = {2017},
	journal={Journal of Parallel and Distributed Computing},
	volume={107},
	pages={37--53},
    issn={0743-7315},
	doi={https://doi.org/10.1016/j.jpdc.2017.04.002}
}

@inproceedings{islam2019toward,
  title={Toward a Programmable Analysis and Visualization Framework for Interactive Performance Analytics},
  author={Islam, Tanzima and Ayala, Alexis and Jensen, Quentin and Ibrahim, Khaled},
  booktitle={2019 IEEE/ACM International Workshop on Programming and Performance Visualization Tools (ProTools)},
  pages={70--77},
  year={2019},
  organization={IEEE}
}

@inproceedings{thiagarajan2018paddle, 
author={Thiagarajan, Jayaraman J.  and Anirudh, Rushil and Kailkhura, Baibhab and Jain, Nikhil and Islam, Tanzima Z. and Bhatele, Abhinav and Yeom, Jae-sung and Gamblin, Todd}, 
booktitle={2018 IEEE International Parallel and Distributed Processing Symposium (IPDPS)}, 
title={PADDLE: Performance Analysis Using a Data-Driven Learning Environment}, 
year={2018}, 
volume={}, 
number={}, 
pages={784-793}, 
keywords={data visualisation;inference mechanisms;learning (artificial intelligence);parallel processing;power aware computing;sparse matrices;complex inference tasks;statistical inferencing;algorithmic solutions;PADDLE;HPC data;information-theoretic approach;hierarchical feature learning;power consumption;machine learning framework;visualization;data-driven learning environment;sparse matrices;Analytical models;Data models;Machine learning;Task analysis;Feature extraction;Performance analysis;Robustness;machine learning;performance data;feature learning;interpretability}, 
doi={10.1109/IPDPS.2018.00088}, 
ISSN={1530-2075}, 
month={May}}

@article{karamizadeh2013overview,
  title={An overview of principal component analysis},
  author={Karamizadeh, Sasan and Abdullah, Shahidan M and Manaf, Azizah A and Zamani, Mazdak and Hooman, Alireza},
  journal={Journal of Signal and Information Processing},
  volume={4},
  number={3B},
  pages={173},
  year={2013},
  publisher={Scientific Research Publishing}
}

@article{davis1999combined,
  title={A combined unifrontal/multifrontal method for unsymmetric sparse matrices},
  author={Davis, Timothy A and Duff, Iain S},
  journal={ACM Transactions on Mathematical Software (TOMS)},
  volume={25},
  number={1},
  pages={1--20},
  year={1999},
  publisher={ACM New York, NY, USA}
}

@inproceedings{bruckstein2008sparse,
  title={Sparse non-negative solution of a linear system of equations is unique},
  author={Bruckstein, Alfred M and Elad, Michael and Zibulevsky, Michael},
  booktitle={3rd International Symposium on Communications, Control and Signal Processing},
  year={2008},
  organization={IEEE},
  pages={762--767},
}

@misc{nvml,
author = Nvidia,
title = {Nvidia Management Library (NVML)},
howpublished={\url{https://developer.nvidia.com/nvidia-management-library-nvml}}
}

@misc{cupti-ref,
  title =  {{CUPTI API Reference}},
  author = {NVIDIA Corp.},
  howpublished = {\url{https://docs.nvidia.com/cuda/cupti/index.html}},
  year={2020}
}

@misc{libnvcd,
  title = {{LibNVCD}},
  howpublished = {\url{https://github.com/tzislam/libnvcd}},
  year={2020}
}

@article{shende2006tau,
  title={The TAU parallel performance system},
  author={Shende, Sameer S and Malony, Allen D},
  journal={The International Journal of High Performance Computing Applications},
  number={2},
  pages={287--311},
  year={2006},
  publisher={Sage Publications Sage CA: Thousand Oaks, CA}
}

@article{adhianto2010hpctoolkit,
  title={HPCToolkit: Tools for performance analysis of optimized parallel programs},
  author={Adhianto, Laksono and Banerjee, Sinchan and Fagan, Mike and Krentel, Mark and Marin, Gabriel and Mellor-Crummey, John and Tallent, Nathan R},
  journal={Concurrency and Computation: Practice and Experience},
  volume={22},
  number={6},
  pages={685--701},
  year={2010},
  publisher={Wiley Online Library}
}

@misc{matmultref,
author = {{Luc Waeijen}},
title = {{Matrix Multiplication CUDA}},
howpublished={\url{https://gitlab.com/ecatue/gpu\_matrixmul\_cuda}},
year={2018}
}

@inproceedings{benjamin2019diogenes,
author = {Welton, Benjamin and Miller, Barton P.},
title = {Diogenes: Looking for an Honest CPU/GPU Performance Measurement Tool},
year = {2019},
isbn = {9781450362290},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3295500.3356213},
doi = {10.1145/3295500.3356213},
abstract = {GPU accelerators have become common on today's leadership-class computing platforms. Exploiting the additional parallelism offered by GPUs is fraught with challenges. A key performance challenge faced by developers is how to limit the time consumed by synchronization and memory transfers between the CPU and GPU. We introduce the feed-forward measurement (FFM) performance tool model that automates the identification of unnecessary or inefficient synchronization and memory transfer, providing an estimate of potential benefit if the problem were fixed. FFM uses a new multi-stage/multi-run instrumentation model that adjusts instrumentation based application behavior on prior runs, guiding FFM to problematic GPU operations that were previously unknown. The collected data feeds a new analysis model that gives an accurate estimate of potential benefit of fixing the problem. We created an implementation of FFM called Diogenes that we have used to identify problems in four real-world scientific applications.},
booktitle = {Proceedings of the International Conference for High Performance Computing, Networking, Storage and Analysis},
articleno = {21},
numpages = {20},
keywords = {performance analysis, performance tools, GPUs, multi-stage/multi-run performance tool design, feed forward measurement},
location = {Denver, Colorado},
series = {SC '19}
}

@INPROCEEDINGS{zhang20122a,
  author={Y. {Zhang} and J. D. {Owens}},
  booktitle={2011 IEEE 17th International Symposium on High Performance Computer Architecture}, 
  title={A quantitative performance analysis model for GPU architectures}, 
  year={2011},
  volume={},
  number={},
  pages={382-393},
}

@INPROCEEDINGS{chen2018towards,
  author={M. {Chen} and I. -. {Chung} and B. {Abali} and P. {Crumley}},
  booktitle={30th International Symposium on Computer Architecture and High Performance Computing (SBAC-PAD)}, 
  title={Towards a Single-Host Many-GPU System}, 
  year={2018},
  volume={},
  number={},
  pages={140-147},} 

@INPROCEEDINGS{bateni2020cooptimizing,
  author={S. {Bateni} and Z. {Wang} and Y. {Zhu} and Y. {Hu} and C. {Liu}},
  booktitle={2020 IEEE Real-Time and Embedded Technology and Applications Symposium (RTAS)}, 
  title={Co-Optimizing Performance and Memory Footprint Via Integrated CPU/GPU Memory Management, an Implementation on Autonomous Driving Platform}, 
  year={2020},
  volume={},
  number={},
  pages={310-323}}

@inproceedings{zhou2018s,
  title={S\^3dnn: Supervised streaming and scheduling for gpu-accelerated real-time dnn workloads},
  author={Zhou, Husheng and Bateni, Soroush and Liu, Cong},
  booktitle={2018 IEEE Real-Time and Embedded Technology and Applications Symposium (RTAS)},
  pages={190--201},
  year={2018},
  organization={IEEE}
}

@inproceedings{boyer2013load,
  title={Load balancing in a changing world: dealing with heterogeneity and performance variability},
  author={Boyer, Michael and Skadron, Kevin and Che, Shuai and Jayasena, Nuwan},
  booktitle={Proceedings of the ACM International Conference on Computing Frontiers},
  pages={1--10},
  year={2013}
}

@phdthesis{delorme2013parallel,
  title={Parallel sorting on the heterogeneous {AMD} fusion accelerated processing unit},
  author={Delorme, Michael Christopher},
  year={2013},
  school={University of Toronto}
}

@inproceedings{zhou2015gpes,
  title={GPES: A preemptive execution system for GPGPU computing},
  author={Zhou, Husheng and Tong, Guangmo and Liu, Cong},
  booktitle={21st IEEE Real-Time and Embedded Technology and Applications Symposium},
  pages={87--97},
  year={2015},
  organization={IEEE}
}

@inproceedings{ganguly2019interplay,
  title={Interplay between hardware prefetcher and page eviction policy in CPU-GPU unified virtual memory},
  author={Ganguly, Debashis and Zhang, Ziyu and Yang, Jun and Melhem, Rami},
  booktitle={Proceedings of the 46th International Symposium on Computer Architecture},
  pages={224--235},
  year={2019}
}

@inproceedings{landaverde2014investigation,
  title={An investigation of unified memory access performance in cuda},
  author={Landaverde, Raphael and Zhang, Tiansheng and Coskun, Ayse K and Herbordt, Martin},
  booktitle={2014 IEEE High Performance Extreme Computing Conference (HPEC)},
  pages={1--6},
  year={2014},
  organization={IEEE}
}

@inproceedings{hestness2015gpu,
  title={GPU computing pipeline inefficiencies and optimization opportunities in heterogeneous CPU-GPU processors},
  author={Hestness, Joel and Keckler, Stephen W and Wood, David A},
  booktitle={2015 IEEE International Symposium on Workload Characterization},
  pages={87--97},
  year={2015},
  organization={IEEE}
}

==> notes.tex <==


% An example of a floating figure using the graphicx package.
% Note that \label must occur AFTER (or within) \caption.
% For figures, \caption should occur after the \includegraphics.
% Note that IEEEtran v1.7 and later has special internal code that
% is designed to preserve the operation of \label within \caption
% even when the captionsoff option is in effect. However, because
% of issues like this, it may be the safest practice to put all your
% \label just after \caption rather than within \caption{}.
%
% Reminder: the "draftcls" or "draftclsnofoot", not "draft", class
% option should be used if it is desired that the figures are to be
% displayed while in draft mode.
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{myfigure}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure}

% Note that the IEEE typically puts floats only at the top, even when this
% results in a large percentage of a column being occupied by floats.


% An example of a double column floating figure using two subfigures.
% (The subfig.sty package must be loaded for this to work.)
% The subfigure \label commands are set within each subfloat command,
% and the \label for the overall figure must come after \caption.
% \hfil is used as a separator to get equal spacing.
% Watch out that the combined width of all the subfigures on a 
% line do not exceed the text width or a line break will occur.
%
%\begin{figure*}[!t]
%\centering
%\subfloat[Case I]{\includegraphics[width=2.5in]{box}%
%\label{fig_first_case}}
%\hfil
%\subfloat[Case II]{\includegraphics[width=2.5in]{box}%
%\label{fig_second_case}}
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure*}


==> results.tex <==

This section presents the analysis for four HPC applications. We target the following questions to identify hardware-application interactions that can explain the average power usage, device utilization, and opportunity for optimizing both device utilization and execution time of applications. 
For each experiment, we varied the execution frequencies on GPUs, the input to each application, and measured the average SM utilization, average power usage, and execution times of several main application kernels.
%%We are interested about application agnostic observations. So we should do an across application characterization. All regions, all input, and all sorts of stuff. 
\begin{itemize}
    \item Which hardware resource utilization and performance events can explain the average power consumption during kernel executions? 
    %We need this for understanding the behavior
    \item Which hardware resource utilization and performance events can explain the loss of device utilization during kernel executions? 
    %%We need this for identifying optimization
    \item Which hardware resource utilization and performance events should be targeted for optimization to improve both device utilization and application performance?
    %\item Identifying the correlation between on-GPU average sm utilization metric and the GPU resource utilization behaviors (as well as hardware performance events) across all applications, all inputs.
    %% to prune the number of cupti events to collect.
\end{itemize}

In this paper, we collect the high-level target metrics (average power usage and average device utilization) through NVML~\cite{nvml} and CUPTI performance events for several computation kernels through source-code annotation tool~\cite{libnvcd}. In addition to collecting per-region execution time, we also compute the score metric presented in Equation~\ref{eqn:score}. 

\input{avgpower}
\input{avgLossSmUtil}
\input{score}
% \input{kripke}
% \input{pennant}
% \input{cloverleaf}

\subsection{Discussion}

\hl{There should be one discussion about -- which resources important for runtime, device utilization separately. Then, we made a join analysis with sparse coding, and that shows which resources are important for joint optimization. Otherwise, it is hard to compare the similarity. }

The interesting observation that can be made from Figure~\ref{fig:sunburst-score} is that the following resource utilization behaviors are important across all four applications ran with four different computation frequencies and several input problems (160 configurations). \hl{What is that one common optimization that we can propose that can help all kernels to reduce L2 utilization?} There are two kernels that will benefit from reducing the bank utilization. Related work~\cite{XX} has identified a common optimization strategy for reducing (or eliminating) bank conflicts by rearranging data structures. For e.g., XX kernel uses array of structures which is not optimal for GPU programming. By rearranging data structures from array of structures to structure of arrays, adjacent threads can access adjacent elements, which will prevent bank conflicts. This optimization will reduce bank conflict (and improve both device utilization and application performance) for several kernels across multiple applications (\texttt{egpuMain4@Pennant}, \texttt{egpuMain5@Pennant}, and \texttt{dot\_kerel@MiniFE}). 

\hl{We should at least show one optimization that improves both device utilization and execution time. Then we can claim this to be true.}
% \begin{itemize}
%     \item Provide a list of CUPTI counters that are always important for power, avgSMUtil, or the ratio.
% \end{itemize}

==> score.tex <==
The objective of this experiment is to identify hardware resource utilization behaviors (and performance events) that can be optimized to improve both GPU device utilization and application performance. For this task, we use the CUPTI hardware performance events to explain the proposed target metric: $1 - normalized\_average\_sm\_utilization/normalized\_execution\_time$. The rationale for using this target metric is that when \texttt{average\_sm\_utilization} is high (good utilization) or application execution time is low (good application performance), the ratio increases. $1-ratio$ computes a quantity that should be minimized to improve either or both of the quantities (device utilization and application performance). 

From Figure~\ref{fig:sunburst-score}, we can make the following observations:
\begin{itemize}
    \item In Figure~\ref{fig:sunburst-score}a, increasing the GPU frequency from 135 MHz to 1530 MHz changes the impact of resources on the utilization and performance ratio. Specifically, all kernels become memory bound at high frequency (L2 at 1530 MHz) from compute bound at low frequency (the number of thread blocks and warps launched at 135 MHz).
    \item In Figure~\ref{fig:sunburst-score}b, the device utilization behavior and the performance of \texttt{egpuMain} is dominated by the 
    \item In Figure~\ref{fig:sunburst-score}c --> Cloverleaf
    \item In Figure~\ref{fig:sunburst-score}d, increasing frequency from 135 MHz to 1530 MHz amplifies the impact of bank conflicts due to load instructions from the shared cache on both device utilization and application performance in the \texttt{dot\_kernel} kernel. 
\end{itemize}



==> tool.tex <==
The measurement tool has two components -- (1) source-code annotation and (2) dynamic library interception. The CUDA Profiling Tools Interface (CUPTI) enables the creation of profiling and tracing tools that target CUDA applications. 
CUPTI provides access to performance events belonging to several categories (called domains). Due to the limited number of performance counter registers, only a subset of the events from each domain can be counted at once. Groups of events that can be measured together 

% An instance of type cupti\_event\_data\_t, which refers to major event
%       counter data and a list of different major metrics.
%  Each major metric refers to its own unique instance of cupti\_event\_data\_t,
%       which in turn holds data references to event counters that the corresponding
% %       metric requires.
%   Each event counter belongs to a specific domain category.
%   Each event counter must be assigned to a specific group at runtime.
%  Groups are necessary for the event counters to actually be counted throughout the execution of a kernel.
%  A group of event counters cannot contain counters from different domains.
%  There is no guarantee that a group can contain all event counters from a domain.
%         Often enough, multiple groups are necessary if an entire domain is to be covered.
 Groups must be explicitly enabled and disabled by the CUPTI API before their counters may be recorded.
  Not all groups can be enabled at once.
  The implication: there's a chance that multiple invocations of the kernel must be performed for all event counters or metrics to be recorded. The \tool provides simple function call that must be set around the user's GPU kernels. The library also uses function call interception to dynamically intercept the API functions and under the hood manage interaction with the CUPTI API. This approach ensures that an application developer who may not be an expert in using CUPTI but still wants to collect fine-grained performance events can do so without much effort. The tool itself has very little dependence on anything else but CUPTI. 
  
  The \tool provides a standalone utility for automatically generating a list of performance events that can be measured together for all available domains on a GPU.
 
%  A simple hooking mechanism is used to wrap around the user's kernel invocation. This allows for the library
%     to internally track which event counters have been computed, and then continuously invoke the same kernel if needed
%     until the desired information has been acquired.
 
 \subsection{Compiler Support}
   NVCC is the compiler used for all source code, both cuda specific and non-cuda specific.
   C++ support is necessary, since cuda source files are C++ - not C.
   NVCC acts as a proxy for gcc; gcc-specific arguments are passed using a specific
      flag `--compiler-options`,  which forwards the arguments as a complete string.
      This is used in many areas, and can be used multiple times throughout the same command.
    NVCC has its own set of nvcc-specific flags, some of which refer to features
      similar to what is available by gcc.
    For .cu files, nvcc -std=c++11 must be passed directly to nvcc,
      but not through the string provided via `--compiler-options`.

\subsection{Usage}

\begin{lstlisting}[language=C++, caption=User-defined granularity]

\_\_global\_\_ void my\_device\_compute\_kernel(...) {\\
    nvcd\_begin(thread_index);\\
    // \\
    // Your device kernel execution code here
    //
    nvcd\_end(thread\_index);
}

\_\_host\_\_ void my\_host\_kernel\_client(...) {
    nvcd\_init();
    my\_device\_compute\_kernel<<param1, param2, ...>>;
    //...
    nvcd\_finalize();
}


\end{lstlisting}

\hl{nvcd device begin() and nvcd device end() are both used to report per-thread information such as runtime, streaming multiprocessor (SM) the thread was executed on, etc.
nvcd host begin() and nvcd host end() are used to allocate device memory as well as cpu-side CUPTI metadata that’s used for tracking various event counters and metrics.
Note that nvcd init() and nvcd terminate() only need to be called once during the execution of the application. nvcd host begin() and nvcd host end() can be called in multiple places. As it stands, the host begin function will currently reallocate all needed memory for computing the desired metrics/event counters for the amount of threads passed. Naturally, the host end function will free said memory.
Eventually, improvements on these capture methods will be provided, but currently the desired metrics and counts are reported to stdout once nvcd host end() is called.}

%\begin{flushleft}
nvcd\_begin() and nvcd\_end() are used to allocate device memory as well
as cpu-side CUPTI metadata that's used for tracking various event counters and metrics.
%\end{flushleft}

%\begin{flushleft}
Note that nvcd\_init() and nvcd\_finalize() only need to be called once during the execution of
the application. nvcd\_begin() and nvcd\_end() can be called in multiple places.
The nvcd\_begin function will currently reallocate all needed memory for computing
the desired performance events for the number of threads being used by the application. The nvcd\_end function will free said memory.
%\end{flushleft}

%\begin{flushleft}
Eventually, improvements on these capture methods will be provided, but currently the desired metrics and
counts are reported to stdout once nvcd\_host\_end() is called.
%\end{flushleft}

\subsection{Environment variables}

\begin{lstlisting}[language=bash, caption=Specifying metrics and event counters through environment variables]
  export BENCH\_EVENTS="l1\_global\_load\_miss:l2\_subp0\_write\_sector\_misses:l2\_subp0\_read\_sector\_misses:active\_warps:branch:divergent\_branch"
  \end{lstlisting}

  Desired metrics and events are specified through bash environment variables. These settings will apply
  to all calls to the nvcd functions. The user may also change the prefix from `BENCH` to anything else they wish.

\subsection{Output Format}

The \tool generates output in CSV format currently. In future, we will implement 
